Hierarchical Agentic Incident Response with Digital-Twin-Validated Attack Inference

Network incident response remains slow and labor-intensive as the defender must infer multi-stage attacks from partial observations and translate recovery decisions into reliable system commands. Decision-theoretic planners provide principled optimization but typically rely on abstract states and predefined actions, while large language model (LLM) agents can reason over operational context but may hallucinate attacks and responses. Toward automating response planning, we present a hierarchical agentic response framework that integrates LLM-based attack inference, rollout planning, and digital-twin validation. A fine-tuned LLM infers the attack progression and affected hosts from security alerts and system measurements. An emulated network digital twin replays the inferred attack and returns discrepancies between predicted and observed effects to calibrate the inference. A separately fine-tuned planning agent uses the rollout planning method to prioritize affected components at the tactical layer. At the operational layer, the planning agent proposes high-level recovery actions, and an execution agent translates selected actions into recovery and verification commands that are validated in the digital twin. We evaluate the framework on a 33-component enterprise-network testbed under three multi-stage attack scenarios. The results show that our framework outperforms frontier-LLM baselines in recovery success rate by 18--31%.

==> tikz/networked_system_component.tex <==
% Digital-twin network component for Fig. 1.
% Four servers and one centered router, drawn directly in the surrounding
% tikzpicture.
%
% Required TikZ libraries in main.tex:
% \usetikzlibrary{arrows.meta,calc,shapes.geometric,shadings}

\definecolor{networkswitch}{HTML}{00A0B5}
\definecolor{networkroutertop}{HTML}{E94B9B}

% Custom 3-D server shape extracted from deployment2.tex.
\makeatletter
\pgfkeys{/pgf/.cd,
  parallelepiped offset x/.initial=2mm,
  parallelepiped offset y/.initial=2mm
}
\pgfdeclareshape{parallelepiped}{
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfmathsetlength\pgfutil@tempdima
      {\pgfkeysvalueof{/pgf/parallelepiped offset x}}
    \pgfmathsetlength\pgfutil@tempdimb
      {\pgfkeysvalueof{/pgf/parallelepiped offset y}}
    \def\ppd@offset{\pgfpoint{\pgfutil@tempdima}{\pgfutil@tempdimb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathclose
    \pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathlineto
      {\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@ya}}{\ppd@offset}}
    \pgfpathlineto
      {\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\ppd@offset}}
    \pgfpathlineto
      {\pgfpointadd{\pgfpoint{\pgf@xa}{\pgf@yb}}{\ppd@offset}}
    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto
      {\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\ppd@offset}}
  }
}
\makeatother

\tikzset{
  network ports/.style={
    line width=0.3pt,
    top color=gray!20,
    bottom color=gray!80
  },
  network server/.style={
    parallelepiped,
    fill=white,
    draw=black,
    minimum width=0.35cm,
    minimum height=0.75cm,
    parallelepiped offset x=3mm,
    parallelepiped offset y=2mm,
    xscale=-1,
    path picture={
      \draw[top color=gray!5,bottom color=gray!40]
        (path picture bounding box.south west) rectangle
        (path picture bounding box.north east);
      \coordinate (network-center) at
        ($(path picture bounding box.center)!0!(path picture bounding box.south)$);
      \coordinate (network-west) at
        ([xshift=-0.575cm]path picture bounding box.west);
      \draw[network ports]
        ([yshift=0.1cm]$(network-west)!0!(network-center)$)
        rectangle +(0.2,0.065);
      \draw[network ports]
        ([yshift=0.01cm]$(network-west)!0.085!(network-center)$)
        rectangle +(0.15,0.05);
      \fill[black]
        ([yshift=-0.35cm]$(network-west)!-0.1!(network-center)$)
        rectangle +(0.235,0.0175);
      \fill[black]
        ([yshift=-0.385cm]$(network-west)!-0.1!(network-center)$)
        rectangle +(0.235,0.0175);
      \fill[black]
        ([yshift=-0.42cm]$(network-west)!-0.1!(network-center)$)
        rectangle +(0.235,0.0175);
    }
  }
}

% Draw the component directly in the surrounding tikzpicture.
% #1 is the center coordinate, e.g. dticon.center.
\newcommand{\drawnetworkedsystemcomponentat}[1]{%
\begin{scope}[shift={(#1)},scale=0.76,transform shape]

  % Background frame centered at (0,0).
  \draw[fill=black!6,line width=0.1mm]
    (-0.55,1.00) rectangle (0.55,-1.00);

  % Four servers symmetric about the central router.
  \coordinate (network-axis) at (0,0);
  \coordinate (server-nw-pos) at (-0.1975, 0.715);
  \coordinate (server-ne-pos) at ( 0.3025, 0.715);
  \coordinate (server-sw-pos) at (-0.1975,-0.785);
  \coordinate (server-se-pos) at ( 0.3025,-0.785);

  % Network links drawn behind the devices.
  \draw[line width=0.14mm,rounded corners=2pt,draw=black]
    (server-nw-pos) -- (server-ne-pos);
  \draw[line width=0.14mm,rounded corners=2pt,draw=black]
    (server-sw-pos) -- (server-se-pos);
  \draw[line width=0.14mm,rounded corners=2pt,draw=black]
    (0,0.715) -- (0,-0.785);

  % Upper and lower server pairs.
  \node[network server,scale=0.35]
    (server-nw) at (server-nw-pos) {};
  \node[network server,scale=0.35]
    (server-ne) at (server-ne-pos) {};
  \node[network server,scale=0.35]
    (server-sw) at (server-sw-pos) {};
  \node[network server,scale=0.35]
    (server-se) at (server-se-pos) {};

  % Centered magenta/cyan router.
  \begin{scope}[shift={(network-axis)},yshift=0.04cm]
    \shade[
      draw=black,
      line width=0.08mm,
      left color=networkswitch,
      right color=white
    ]
      (-0.18,0.00)
      arc[
        start angle=180,
        end angle=360,
        x radius=0.18,
        y radius=0.055
      ]
      -- (0.18,-0.08)
      arc[
        start angle=360,
        end angle=180,
        x radius=0.18,
        y radius=0.055
      ]
      -- cycle;

    \shade[
      draw=black,
      line width=0.08mm,
      left color=networkroutertop,
      right color=networkroutertop!20!white
    ]
      (0,0) ellipse [x radius=0.18,y radius=0.055];

    % Four-direction router mark.
    \begin{scope}[yscale=0.35]
      \foreach \Angle in {0,90,180,270}{
        \draw[
          white,
          line width=0.05mm,
          -{Latex[length=0.25mm,width=0.20mm]}
        ]
          (0,0) -- (\Angle:0.10);
      }
    \end{scope}
  \end{scope}

\end{scope}
}
